Pomset logic: the other approach to non commutativity in logic

Thirty years ago, I introduced a non-commutative variant of classical linear logic, called "pomset logic", issued from a particular categorical interpretation of linear logic known as coherence spaces. In addition to the usual commutative multiplicative connectives of linear logic, pomset logic includes a non-commutative connective, "$\triangleleft$" called "before", associative and self-dual: $(A\triangleleft B)^\perp=A^\perp \triangleleft B^\perp$. The conclusion of a pomset logic proof is a Partially Ordered MultiSET of formulas. Pomset logic enjoys a proof net calculus with cut-elimination, denotational semantics, and faithfully embeds sequent calculus. The study of pomset logic has reopened with recent results on handsome proof nets, on its sequent calculus, or on its following calculi like deep inference by Guglielmi and Strassburger. Therefore, it is high time we published a thorough presentation of pomset logic, including published and unpublished material, old and new results. Pomset logic (1993) is a non-commutative variant of linear logic (1987) as for Lambek calculus (1958!) and it can also be used as a grammatical formalism. Those two calculi are quite different, but we hope that the algebraic presentation we give here, with formulas as algebraic terms and with a semantic notion of proof (net) correctness, better matches Lambek's view of what a logic should be.

==> LatexPackages/INSTALL <==
THE ST MARY'S ROAD SYMBOL FONT

6 APRIL 1994

This distribution contains the St Mary's Road symbol fonts:

   INSTALL       stmary5.mf    stmary8.mf    stmaryba.mf   stmaryrd.dtx
   README        stmary6.mf    stmary9.mf    stmarych.mf   stmaryrd.mf
   stmary10.mf   stmary7.mf    stmaryaj.mf   stmaryjg.mf

To install the fonts, you should:

 * run METAFONT on the fonts, for example under Unix you say:

      mf "\mode=localfont; input stmary5;"
      mf "\mode=localfont; input stmary6;"
      mf "\mode=localfont; input stmary7;"
      mf "\mode=localfont; input stmary8;"
      mf "\mode=localfont; input stmary9;"
      mf "\mode=localfont; input stmary10;"

 * move stmary*.tfm into a TeX font metrics directory

 * move stmary*.*pk into a TeX bitmaps directory

If you want to use the St Mary's Road font in LaTeX2e, you should:

 * run LaTeX2e on stmaryrd.dtx

 * move stmaryrd.sty and Ustmry.fd into a TeX inputs directory

 * read the documentation in stmaryrd.dvi

This file should only be distributed as part of the St Mary's Road
distribution.

Copyright 1994 Alan Jeffrey


==> LatexPackages/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O�Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...�': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> dechets.tex <==
As indicated in Section \ref{dicographs} we write $a\--b$ for the edge or par of opposite arcs $(a,b),(b,a)$

\begin{example}{Example $\ts\pa4$ } 
Here is a correct proof net that rewrites to a correct proofnet using $\ts\pa4$: 


$B=\{a\edge a^\perp, b\edge b^\perp, c\edge c^\perp, d\edge d^\perp\}$

$R=(a^\perp\tssp b^\perp)\pasp  ((a\pasp b)\tssp (c\pasp d)) \pa c^\perp\pa d^\perp=
\{a^\perp\edge b^\perp, b\edge c, b\edge d, a\edge c, a\edge d\}$

$R'=(a^\perp\tssp b^\perp)\pasp  ((a\tssp c)\pasp (b\tssp d)) \pa c^\perp\pa d^\perp=
\{a^\perp\edge b^\perp, b\edge c, b\edge d, a\edge c, a\edge d\}$

$(B,R)$ is correct, and using $\ts\pa4$ it rewrites to $(B,R')$
which is correct as well. 
\end{example} 

It is also easy to find an incorrect proof structure that rewrites into a correct proof structure using a rewriting rule that preserves correctness, e.g. $(V,B=a\edge a^\perp,R=a\befsp a^\perp)$ whch rewrites to 
$(V,B=a\edge a^\perp,R=a \pasp a^\perp)$ sing $\bef\pa2$



and at the end of $d^1$ and which is replaced with 
(with an external $\ts(a_i\pa a_i^\perp)$ repeated at the end of each dicograph in the derivation, 
 
is replaced with a $\un$ by a tensor to the axiom the SBV  derivation, a $\un$ that is immediately turned into  $a_i\pa a_i^\perp$. We then apply n first steps of $d_{pom}$, the . Then, as proposition \ref{internalise} shows we can move the $a_i\pa a_i^\perp$ to the place of the $\un$ in the dicograph, then we do the SVB 




\begin{proof} 
The derivation can ``almost" be mimicked step by step. 

One little difference concerns axioms. In SBV axioms are $\un$ that appears to start with or anywhere inside the dicographs at any point of the derivation. Some of those $\un$ are turned into $a_k\perp a_k^\perp$ while some remain. 


The $\un$ that appear somewhere in the derivation and that do not vanish must be anticipated as axioms $\epsilon\pa \epsilon^\perp$ in the deep pomset derivation. 

The proof should be clear for any one familiar with SBV,  deep inference and the like; instead of a lenghty  formal proof let us give arguments that bring enough evidence. 

\noindent\underline{From SBV derivations to deep pomset derivation:}  
Equalities (associativity, commutativity, singleton, contextual closure) are for us plain  equalities that need not equations in deep pomset. 


Firstly, one can get rid of $\un$ that appear and finally disappear --- any formula can be traced in a multiplicative proof or rewriting like SBV or deep pomset. 

Let us trace in the SBV derivation the appearance of $\un$ and let us follow each $\un$ in the derivation up to the point where it is replaced by $a_i,a_i^\perp$. We proceed by induction on the number of $\un$ that appear before being replaced by some $a_i,a_i^\perp$. 
The SBV derivation up to the appearance of the first  $\un$ has no $\un$, to we have a deep pomset derivation, say $d$, yielding to $t$, which is the same as the SBV derivation.  
At the beginning of $d$  we add a $\un$ linked by a tensor immediately turning into an axiom $a_i \pasp a_i^\perp$ with the initial axiom, i.e. we add it as a tensor of the initial axiom. The BV derivation goes on, with this axiom linked via a tensor link up to the point where the $\un$ appears. At this point, instead of pursuring the SBV derivation $d$, we move the $a_i \pasp a_i^\perp$ inside the term at the precise place where the $\un$ appears. 
Then we pursue the SBV derivation with $a_i \pasp a_i^\perp$ in place of $\un$, up to the point where the $\un$ was replaced with $a_i \pasp a_i^\perp$. 
In this SBV derivation, we have one $\un$ that appears and disappears less. 


$\un$ in pomset logic simply is an axiom, a B-edge with one vertex called $\un$ whose other vertex is pendent, not incident to any R edge of the dicograph --- one may callthis vertex $i$.  
Never can an \ae-cycle pass through this axiom or B edge. 


\noindent\underline{From deep pomset derivation to SBV derivation:}  The other direction is completely straightforward:
one should just observe that the rules $a\downarrow$
and Unit for tensor allow to derive the deep pomset axiom: there after all rules of deep pomset are SBV rules. 
\end{proof} 


\begin{theorem}\label{sbv1} 
Any SBV derivation, possibly with $\un$ in its conclusion, can be mapped into a deep pomset derivation with $\un$ and vice versa. 
\end{theorem} 


\begin{proof} 

\end{proof} 






The main difference is $\un$
\begin{itemize} 
\item 
The axiom of SBV is simply $\un$. As there are no more $\un$ by the end of the derivation, it means all $\un$ have been replaced with $a,a^\perp$ for a propositional letter $a$ during the derivation, or that they vanished.
\item 
Observe that some $\un$ may pop in any where in a dicograph, and then move to some place according to the structural rules of SBV before being substituted with an axiom. 
\end{itemize} 


As said above, cuts are simply subterms of the form $K\tssp K^\perp$ such that the connectives that dominate  this $\tssp$ in the term (the connective closer to the root when the term is viewed as a tree)
never are $\tssp$ (can only be $\befsp$ or $\pasp$).\footnote{It is possible in this calculus with dicographs of atoms as sequents to embed a cut inside any formula,  ie that the cut is dominated other tensors, and possibly by cuts, but this seems far beyond what is presently understood about pomset logic.} 


\begin{prooftree} 
\seq \Gamma \pasp X [I] \qquad  \seq X^\perp,\Delta [J] 
\justifies 
\seq \Gamma,\Delta [I \lts{X,X^\perp} J |_{\Gamma,\Delta}]
\using cut 
\end{prooftree} 




A similar inductive of irreflexive binary relation is the class of cographs: 
the empty relation over a singleton domain is a cograph. 
Given two graphs  $R_1\subset (E_1)^2$ and $R_2\subset (E_2)^2$  over two disjoint finite sets $E_1$ and $E_2$ 
let us define their symmetric series composition $R_1\tssp R_2$ with domain $E_1\uplus E_2$ as  $R_1\uplus R_2 \uplus E_1\times E_2 \uplus E_2\times E_1$. 
Cographs are the smallest class of binary relations closed under symmetric series composition and parallel composition. This class of graph is characterised by the absence of $P_4$ as an induced subgraph on four points. 


%%%%%%%

Tensor glueing : given tow sp orders, $O_1$  on $\Gamma_1, A_1$ and and $O_2$ on $\Gamma_2, A_2$  with both $A_1$
and $A_2$ absolute maximum (resp absolute minimum) in a connected component of their respective orders, we define $O_1 \otimes_{A_1\ts A_2} O_2$ as follows. 
If $A_1$ is a minimum  in its connected component of $O_1$ it means that $O_1$ can be written $(A_1\befsp T_1)\pasp U_1$. 
If $A_2$ is a minimum  in its connected component of $O_2$ it means that $O_2$ can be written $(A_2\befsp T_2)\pasp U_2$. Then $O_1 \otimes_{A_1\ts A_2} O_2$ is $((A_1\ts A_2)\befsp (T_1\pasp T_2)) \pasp U_1 \pasp U_2$. 
When $A_1$ and $A_2$ are both maximum in the component of its respective order, 
$O_1$ can be written $(T_1\befsp A_1)\pasp U_1$ $O_2$ can be written  $(T_2\befsp A_2)\pasp U_2$ 
and $O_1 \otimes_{A_1\ts A_2} O_2$ is 
$((T_1\pasp T_2) \befsp    (A_1\ts A_2)) \pasp U_1 \pasp U_2$. 


Times is the usual rule on the formulas, it only applies when the premises are both minimums of their respective components). 

$$
\begin{prooftree} 
\seq (A_1\befsp T_1)\pasp U_1 \qquad \seq (A_2\befsp T_2)\pasp U_2 
\justifies 
\seq ((A_1\ts A_2)\befsp (T_1\pasp T_2)) \pasp U_1 \pasp U_2
\using \ts
\end{prooftree} 
$$


This kind of tensor rule is an adaptation of the rule in \cite{Ret93}, but it is adapted to  sp partial order. \footnote{Actually the condition in \cite{Ret93} was quite complicated. It was relying on the fact that the partial order should be orthogonal to all possible paths in the proof nets, just assuming that it was so to the two smaller proof nets corresponding to the premise. here the condition, $A$ and $B$
being both absolute maximums in their connected components makes sure that there is no cycle but also that the resulting partial order is an sp order.} 

Remark: we could have opted for the rule when $A_1$ and $A_2$ are both maximums in their respective connected components. 
However in order to have cut elimination between a $\pa$ and a $\ts$, but we cannot have both the rules using maximums and minimums, this has to be uniform. 

$$
\begin{prooftree} 
\seq (T_1\befsp A_1)\pasp U_1 \qquad \seq (T_2\befsp A_2)\pasp U_2 
\justifies 
\seq ((T_1\pasp T_2) \befsp    (A_1\ts A_2)) \pasp U_1 \pasp U_2
\using \ts
\end{prooftree} 
$$

%%%%%%%%%%%%%%%%%%%
CALCUL DES SEQUENTS STANDARD 


\section{A sequent calculus in standard style} 

\subsection{Guidelines} 

As discussed in an old paper of mine with François Lamarche \cite{LR96} in order to have a non commutative system, one needs some additional structure on the sequent: a total order for the Lambek calculus (the comma on the right and side is then the non commutative disjunction). 


When the logic is non commutative, the multi set of formulas ought to be endowed with some structure in order to draw a distinction between 
$\seq Gamma, A*B$ and $\seq Gamma, B*A$. Observe that if a  connective is non commutative so is its dual, when the double dual is the initial formula. 

and one of them has a unary rule. Hence there should exists a distinction 
between $\seq Gamma, A, B$ and $\seq Gamma, B, A$, so there should exists some additional structure on the multiset of formulas. 

For non commutativity in the Lambek Abrusci style, the structure is a total cyclic order (ternary relation) or a total order in the intuitionnistic case --- this is similar, because an intuitionistic sequent is a sequent with a chosen output. 




If for some reason we want to extent multiplicative linear logic with a non commutative multplicative connective rather than to restrict existing connective to be non commutative, and want to be minimal why not introducing a single connective, hence selfdual, which would correspond in the partial order to $A<B$ and $A$ and $B$ have the same relation with other formulas? And why not having $(A<B)^\perp\equiv A^\perp < B^\perp$ (instead  of the more common $B^\perp < A^\perp$).
That way one may think of an order on computations: a cut between $(A<B)^\perp$ and $A^\perp < B^\perp$ reduces to two smaller cuts $A--cut--A\perp$ and $B--cut--B\perp$ with the cut on $A$ being  prior to the cut on $B$. This makes sense when linear logic proofs are viewed as programs and cut-elimination as computation. 

Doing so one may obtain a sequent calculus using partially ordered multi sets of formulas. 
One may think of the order as conditions that are met by the occurrences of formulas and in this sense it is natural to have an entropy rule saying that $\seq Gamma$ with some order entails $\Gamma$ in any weaker order. 

A natural structure is a partial order and if one wants every sequent to be equivalent to a single formula, this lead us to series parallel partial orders that are inductively defined by parallel composition (noted $\pasp$) and series composition (noted $\befsp$). 


\subsection{Foreword on sp pomsets}

Given two partial orders $O_1\subset (E_1)^2$ and $O_2\subset (E_2)^2$  over two disjoint finite sets $E_1$ and $E_2$ 
their series composition is $O_1\befsp O_2$ is $O_1\uplus O_2 \uplus E_1\times E_2$
and their parallel composition  $O_1\pasp O_2$ is $O_1\uplus O_2$.
The class of series parallel partial orders is defined from empty orders over singletons. 

Such orders are characterised by the absence of $N$ in the Hasse diagram, or more formally, and sp order restricted to four points $a,b,c,d$  never is $a\befsp b, a'\befsp b, a'\befsp b'$ (up to isomorphism).\cite{Moh89,Moh85,LTV82,BGR97}. 

Series parallel partial order can  be described by an sp term, where each point of the domain appears exactly once; for a given sp order, the sp term is unique up to the commutativity of $\pa$ and to the associativity of both $\pasp$ and $\befsp$. 

Two points $a$ and $b$ are said to be equivalent in an sp order (notation $a \simpa b$) whenever the term can be written (using associativity of $\pasp$ and $befsp$ and the commutativity of $\pasp$)  $T[a\pasp b]$ (one can also say: $a\notbefsp b$, $b\notbefsp a$ and for all $x\neq a,b$ in the domain $a\befsp x$ iff $b\befsp x$ and $x\befsp a$ iff $x\befsp b$. 

Two points $a$ and $b$ are said to be lower equivalent in an sp order (notation) $a \simbef b$ whenever the term can be written (using associativity of $\pasp$ and $\befsp$ and the commutativity of $\pasp$)  $T[a\bef b]$ (one can also say: $a\befsp b$  and for all $x\neq a,b$ in the domain $a\befsp x$ iff $b\befsp x$ and $x\befsp a$ iff $x\bef b$. 




\subsection{Sequent calculus rules} 

In this classical calculus sequents are righthanded, and this single multiset of formulas is endowed with an sp order. One can represent this multiset of formulas endowed with an sp order by an sp term whose atoms are the formulas (and such a term is unique up the commutativity of $\pasp$ and the associativity of $\pasp$ and $\befsp$. 

%Because $A$ and $B$ are both maximal (or minimal), this union is an order, there is no transitive closure to be applied, no cycle, and no induced $N$: so $O_1 \otimes_{A\ts B} O_2$ is an sp order when $O_1$ and $O_2$ are sp orders, and $A-1$ and $A_2$ are absolute maximums (resp minimums) of their connected component in their order. 


\subsection{Structural rules: mix and entropy} 

One rule is needed to introduce some order: it can be called directed MIX:
$$
\begin{prooftree} 
\seq T \qquad \seq S 
\justifies 
\seq T\befsp S 
\using \mbox{\footnotesize MIXSP}  
\end{prooftree} 
$$

and as said above, if the order is viewed as constraints it is natural to have an entropy rule. 


$$
\begin{prooftree} 
\seq T 
\justifies 
\seq T'
\using Entropy — T'\subset T 
\end{prooftree} 
$$ 

As done in \cite{BGR97} $T'\subset T$ is equivalent to $T\rightsquigarrow T'$ using the rewrite rules in figure \ref{inclusionsp} that are defined up to commutativity of $\pasp$ and to the associativity of $\pasp$ and $\befsp$. 


\begin{figure} 
\hrulefill 
\label{inclusionsp} 
$$
\begin{array}{l@{\qquad\qquad}ccccccc @{\qquad}c @{\qquad}cccccccc} 
\bef\pa4 & (X&\pasp& Y)  &\befsp& (U &\pasp& V) & \rightsquigarrow &(X &\befsp& U) &\pasp& (Y&\befsp& V)\\ 
\bef\pa3l& (X&\pasp& Y)  &\befsp& U & & & \rightsquigarrow &(X &\befsp& U) &\pasp& Y & & \\ 
\bef\pa3r &&& Y &\befsp& (U &\pasp& V) & \rightsquigarrow &  && U &\pasp& (Y &\befsp& V)\\ 
%(X\pasp Y)  &\befsp& (U \pasp V) & \rightsquigarrow &(X \befsp U) &\pasp& (Y\befsp V)\\ 
\bef\pa2  & && Y  &\befsp& U &&  & \rightsquigarrow & && U &\pasp& Y && \\ 
\end{array} 
$$ 
\caption{An sp order described by a term $T'$ is included in an sp order $T$if and only if  $T$ rewrites to $T'$ with these rules defined up to 
that are defined up to commutativity of $\pasp$ and to the associativity of $\pasp$ and $\befsp$.} 
\hrulefill 
\end{figure} 


\subsection{Par rule} 

The par rule is unchanged and as one may expect, the par of two formulas correspond to two conclusions that are at equivalent places in the order, none being prior to the other: 
$$
\begin{prooftree} 
\seq T[A\pasp B]
\justifies 
\seq T[A\pa B]
\using \pa 
\end{prooftree} 
$$


\subsection{Before rule} 

The $\bef$ rule is as the par-rule, the two formulas have to be one before the other. 
$$
\begin{prooftree} 
\seq T[A\befsp B]
\justifies 
\seq T[A\bef B]
\using \bef 
\end{prooftree} 
$$

\subsection{Tensor rule and cut rule} 

We knows how the tensor rule behaves wrt formulas. The only aspect that deserves some tuning, is the order on the formulas after applying the rule. Our choice is guided by two independent criteria:
\begin{enumerate} 
\item 
The  resulting partial order should be an sp order. 
\item This sequent calculus should enjoy cut elimination, i.e. when there is a cut between $A\ts B$ and $A^\perp \pa B^\perp$  with $A\ts B$ coming immediately from a $\ts$ rule from $\seq \Gamma, A$ and $\seq \Delta, B$  and $A^\perp \pa B^\perp$  coming immediately from a $\pa$ rule from $\Theta, A^\perp, B^\perp$ one should be able to locally turn those rules into 
two consecutive cuts, one between  $\Theta, A, B$ and $\seq \Gamma, A$ and then one with $\seq \Delta, B$. 
\item This sequent calculus should enjoy cut elimination, i.e. when there is a cut between $A\bef B$ and $A^\perp \bef B^\perp$  with $A\bef B$ coming immediately from a $\bef$ rule from $\seq \Gamma, A, B$  and $A^\perp \bef B^\perp$  coming immediately from a $\bef$ rule from $\seq                                  \Theta, A^\perp, B^\perp$ one should be able to locally turn those rules into 
two consecutive cuts, one between  $\Theta, A, B$ and $\seq \Gamma, A$ and then one with $\seq \Delta, B$. 
\end{enumerate} 



\subsection{Cut rule} 

The cut rule is a particular king of tensor rule, between $K$ and $K^\perp$, yielding $K\times K^\perp\eqiiv \bot$ which is the unit w.r.t. $\pa$. 
A opposed to standard calculus it makes sense that cuts remain within the order between formulas, because the partial order on formulas may be used to reduce them in a given order.



$$
\begin{prooftree} 
\seq (K\befsp T_1)\pasp U_1 \qquad \seq (K^\perp \befsp T_2)\pasp U_2 
\justifies 
\seq (cut \befsp (T_1\pasp T_2)) \pasp U_1 \pasp U_2
\using \ts
\end{prooftree} 
$$



As usual in the multiplicative case, there is little to say about cut-elimination, which is a rather trivial process, because the base cases replace one cut on a formula of size $p$ by two cuts on formulas whose size is strictly smaller than $p$. 
The only point one has to be careful about is the preservation of the order between formulas and cuts. 

here are the basic cases of cut elimination: 

$\pa/\ts$ 




$\bef/\bef$ 



\section{Another sequent calculus prefiguring deep inference} 



==> foldingSequent.tex <==


\subsection{Folding and unfolding pomset logic sequents} 


A structured sequent of pomset logic (resp. of MLL) is a multi set of formulas of pomset logic (resp. of MLL)  with the connectives $\bef,\ts,\pa$ endowed with a dicograph. On such sequents one may define:  
\begin{description} 
\item[\bf Folding]  given a multi set of formulas $X_1,\ldots, X_n$ endowed with a dicograph $T$,
\begin{description} 
\item[$\pa$] if $X_i\simpa X_j$ in $T$ rewrite $T[X_i\pasp X_j]$ into $T[(X_i\pa X_j)]$ --- in the mutiset, $X_i$ and $X_j$ have been replaced with $X_i\pa X_j$. 
\item[$\bef$] if $X_i\simbef X_j$ in $T$ rewrite $T[X_i\befsp X_j]$ into $T[(X_i\bef X_j)]$ --- in the mutiset, $X_i$ and $X_j$ have been replaced with $X_i\bef X_j$. 
\item[$\ts$] if $X_i\simts X_j$ in $T$ rewrite $T[X_i\tssp X_j]$ into $T[(X_i\ts X_j)]$ --- in the mutiset, $X_i$ and $X_j$ have been replaced with $X_i\ts X_j$. 
\end{description}
\item[\bf Unfolding] is the opposite: 
\begin{description} 
\item[$\pa$] turn $T[(X_i\pa X_j)]$  into $T[X_i\pasp X_j]$  --- in the mutiset, $X_i\pa X_j$ has been replaced with two formulas $X_i$ and $X_j$ with $X_i\simpa X_j$
\item[$\bef$] turn $T[(X_i\bef X_j)]$  into $T[X_i\befsp X_j]$  --- in the mutiset, $X_i\pa X_j$ has been replaced with two formulas $X_i$ and $X_j$ with $X_i\simbef X_j$
\item[$\ts$] turn $T[(X_i\ts X_j)]$  into $T[X_i\tssp X_j]$  --- in the mutiset, $X_i\pa X_j$ has been replaced with two formulas $X_i$ and $X_j$ with $X_i\simbef X_j$ 
\end{description}
\end{description} 


==> pomset_cographs.tex <==
% rules for pomset logic 
% the "largest" system

\begin{prooftree} 
\justifies 
\seq a, a^\perp 
\end{prooftree} 

\bigskip 

\begin{prooftree} 
\seq \Gamma, \Theta \qquad  \seq \Phi,\Delta
\justifies 
\seq \Gamma,\langle\Theta,\Phi\rangle,\Delta
\using \timesctxt
\end{prooftree} 
\qquad 
\begin{prooftree} 
\seq \Gamma \qquad  \seq \Delta
\justifies 
\seq (\Gamma;\Delta)
\using dimix
\end{prooftree} 

\bigskip 

\begin{prooftree} 
\seq \Gamma
\justifies 
\seq \Gamma'
\using entropy  (\Gamma \rightsquigarrow \Gamma')
\end{prooftree} 
 
\bigskip 

\begin{prooftree} 
\seq \Gamma[\{A,B\}]
\justifies 
\seq \Gamma[A\pa B]
\using \pa
\end{prooftree} 
\qquad 
\begin{prooftree} 
\seq \Gamma[(A;B)]
\justifies 
\seq \Gamma[A\prec B]
\using \prec 
\end{prooftree} 
\qquad
\begin{prooftree} 
\seq \Gamma[\langle A,B \rangle]
\justifies 
\seq \Gamma[A\lts B]
\using \lts 
\end{prooftree}

\bigskip 


\begin{prooftree} 
\seq \Gamma, K \qquad  \seq K^\perp,\Delta
\justifies 
\seq \Gamma,\Delta
\using cut
\end{prooftree} 


==> pomset_rules.tex <==
% rules for pomset logic 
% the "largest" system

\begin{prooftree} 
\justifies 
\seq a, a^\perp 
\end{prooftree} 

\bigskip 

\begin{prooftree} 
\seq \Gamma, \Theta \qquad  \seq \Phi,\Delta
\justifies 
\seq \Gamma,\langle\Theta,\Phi\rangle,\Delta
\using \timesctxt
\end{prooftree} 
\qquad 
\begin{prooftree} 
\seq \Gamma \qquad  \seq \Delta
\justifies 
\seq (\Gamma;\Delta)
\using dimix
\end{prooftree} 

\bigskip 

\begin{prooftree} 
\seq \Gamma
\justifies 
\seq \Gamma'
\using entropy  (\Gamma \squigarrow \Gamma')
\end{prooftree} 
 
\bigskip 

\begin{prooftree} 
\seq \Gamma[\{A,B\}]
\justifies 
\seq \Gamma[A\pa B]
\using \pa
\end{prooftree} 
\qquad 
\begin{prooftree} 
\seq \Gamma[(A;B)]
\justifies 
\seq \Gamma[A\prec B]
\using \prec 
\end{prooftree} 
\qquad
\begin{prooftree} 
\seq \Gamma[\langle A,B \rangle]
\justifies 
\seq \Gamma[A\lts B]
\using \lts 
\end{prooftree}

\bigskip 


\begin{prooftree} 
\seq \Gamma, K \qquad  \seq K^\perp,\Delta
\justifies 
\seq \Gamma,\Delta
\using cut
\end{prooftree} 

